Accelerating Vision Transformers Based on Heterogeneous Attention Patterns

Recently, Vision Transformers (ViTs) have attracted a lot of attention in the field of computer vision. Generally, the powerful representative capacity of ViTs mainly benefits from the self-attention mechanism, which has a high computation complexity. To accelerate ViTs, we propose an integrated compression pipeline based on observed heterogeneous attention patterns across layers. On one hand, different images share more similar attention patterns in early layers than later layers, indicating that the dynamic query-by-key self-attention matrix may be replaced with a static self-attention matrix in early layers. Then, we propose a dynamic-guided static self-attention (DGSSA) method where the matrix inherits self-attention information from the replaced dynamic self-attention to effectively improve the feature representation ability of ViTs. On the other hand, the attention maps have more low-rank patterns, which reflect token redundancy, in later layers than early layers. In a view of linear dimension reduction, we further propose a method of global aggregation pyramid (GLAD) to reduce the number of tokens in later layers of ViTs, such as Deit. Experimentally, the integrated compression pipeline of DGSSA and GLAD can accelerate up to 121% run-time throughput compared with DeiT, which surpasses all SOTA approaches.

==> ablation_study_glad_version2.tex <==
\subsection{Ablation Studies on GLAD}
% \subsubsection{Analysis of Components within GLAD}
% \noindent{\textbf{Analysis of Components within GLAD.}}
% We deliberately design GLAD, which contains many components including BatchNorm, GeLU, position re-embedding, token distill loss. 
% We make detailed ablation study of these components with respect to Integrated-Deit-S, which serves as baseline model. 

% % LayerNorm and GeLU can stabilize the training and introduces additional non-linearity, respectively.  Position re-embedding makes the spatial information of transformed features distinguished. Token distill loss helps the training of the compressed ViT. 

% As  shown in Tab.~\ref{tab:ablation_GLAD}, 
% the accuracy of configurations without each component is lower than 
% that of the baseline model.
% % The baseline model yeilds +0.3\% Top-1
% %  accuracy in relation to the configuration without BatchNorm and GeLU, which indicates the effectiveness of them. 
%  There is \bp{some improvements} of 0.3\%, 0.2\% and 0.2\% Top-1
%  accuracy by using LayerNorm+GeLU, position re-embedding and token distill. 
% The results indicate the effectiveness of each component. \deli{Moreover, the usage of BatchNorm and GeLU is necessary, since their removings make the training diverge.}  

  

% \begin{table}[htp]
%   \begin{center}
%         \caption{The ablation studies of GLAD w.r.t Integrated-Deit-S}
%       \label{tab:ablation_GLAD}
%       \footnotesize
%   \begin{tabular}{|l|c|}
%   \hline
%   Ablation  & Top-1 Acc. (\%)  \\
%   \hline
%   baseline model & 79.9 \\
%   without LayerNorm+GeLU &  79.6   \\
%   without position re-embedding & 79.7\\
%   without token distill & 79.7\\
%   \hline
%   without self-supervised distill & 79.2\\ 
%   \hline
%  \end{tabular}
%  \end{center}
%  \vspace{-15pt}
%  \end{table}
 


% \subsubsection{Comparison with Other Methods}
In this part, we compare GLAD with other pruning-based and aggregation-based methods to illustrate the effectiveness of GLAD.


\noindent{\textbf{Comparison with pruning-based methods.}} As shown in Tab.~\ref{tab:benchmark}, GLAD-based compression outperforms other pruning-based methods, such as Evo~\cite{xu2021evo}, PS~\cite{tang2021patch}and DynamicViT~\cite{rao2021dynamicvit}, in terms of throughput and accuracy on Deit-Small.
The reasons may come from two folds: 1) pruning-based methods will \bp{lose} spatial information after reducing token numbers, while GLAD can preserve the information as much as possible while reducing token spatial size by a linear aggregation. 2) GLAD is more efficient in run-time mode due to no need of  importance score prediction module which is adopted by DynamicViT~\cite{rao2021dynamicvit} during inference. 
% full number of tokens into less number by 
% The GLAD-based compression is a fair counterpart of other pruning-based methods, . GLAD-Deit-B, GLAD-Deit-S and GLAD-Deit-T produces much higher throughput and less accuracy drop than them. That verifies the effectiveness of GLAD. 

% To thoroughly validate the effectiveness of GLAD, 
\noindent{\textbf{Comparison with aggregation-based methods.}} We also make controlled comparison experiments to compare GLAD with other aggregation-based methods, such as the local concatenation used in Swin~\cite{liu2021swin} and Twins~\cite{chu2021twins}, and down-sampling used in \cite{wu2021cvt}. 

% To make fair comparison, we control the same aggregated token numbers and do not use DGSSA method in the early layers in all experiments.
% We replace GLAD with these methods in Our-Deit-S, respectively. 
 
 \begin{table}[htp]
  \begin{center}
        \caption{The comparison of GLAD with other aggregation-based methods of reducing token spatial size.  }
      \label{tab:comparison_GLAD}
      \footnotesize
  \begin{tabular}{|l|c|c|c|}
  \hline
  Methods & Scope & Ratio & Top-1 Acc.(\%)   \\
  \hline
  GLAD & global  & \textit{flexible} & 79.3 \\
  GLAD & global  & $\frac{1}{4}$ & - \\
  \hline
  concatenation~\cite{liu2021swin,chu2021twins} & local $2 \times 2$ & $\frac{1}{4}$   & 79.2  \\
  down-sampling~\cite{wu2021cvt} & local $2 \times 2$&   $\frac{1}{4}$   & - \\
  \hline
 \end{tabular}
 \end{center}
  \vspace{-15pt}
 \end{table}
 
 As shown in Tab.~\ref{tab:comparison_GLAD}, GLAD outperforms concatenation and down-sampling methods.
 Two features of ``global'' and ``flexible'' may account for the performance.
 1)
%  That may result from that 
Global GLAD has improvement of {x \% and x \% Top-1 accuracy} over local concatenation and down-sampling methods 
with reduction ratio $\frac{1}{4}$  of token number, respectively.
% The feature of ``global'' may account for the performance. 
That indicates the advantage of global scope. 
2) Moreover, the improvement further comes to  0.x \% and 0.x \%   when GLAD flexibly \bp{uses} proper compression configuration of slimmed token number. 
That indicates the effectiveness of flexible aggregation.
% The two local methods aggregate tokens to get less token numbers  within a fixed-size window, such as $2\times 2$.  
% The pre-defined fixed size may not 
% be suitable for the real distribution of feature redundancy information. 
Above all, the comparison results validate the \textit{effectiveness of GLAD which flexibly makes global aggregation.}


